Scalable Biophysical Simulations of the Neuromuscular System

The human neuromuscular system consisting of skeletal muscles and neural circuits is a complex system that is not yet fully understood. Surface electromyography (EMG) can be used to study muscle behavior from the outside. Computer simulations with detailed biophysical models provide a non-invasive tool to interpret EMG signals and gain new insights into the system. The numerical solution of such multi-scale models imposes high computational work loads, which restricts their application to short simulation time spans or coarse resolutions. We tackled this challenge by providing scalable software employing instruction-level and task-level parallelism, suitable numerical methods and efficient data handling. We implemented a comprehensive, state-of-the-art, multi-scale multi-physics model framework that can simulate surface EMG signals and muscle contraction as a result of neuromuscular stimulation. This work describes the model framework and its numerical discretization, develops new algorithms for mesh generation and parallelization, covers the use and implementation of our software OpenDiHu, and evaluates its computational performance in numerous use cases. We obtain a speedup of several hundred compared to a baseline solver from the literature and demonstrate, that our distributed-memory parallelization and the use of High Performance Computing resources enables us to simulate muscular surface EMG of the biceps brachii muscle with realistic muscle fiber counts of several hundred thousands. We find that certain model effects are only visible with such high resolution. In conclusion, our software contributes to more realistic simulations of the neuromuscular system and provides a tool for applied researchers to complement in vivo experiments with in-silico studies. It can serve as a building block to set up comprehensive models for more organs in the musculoskeletal system.

==> document/doc.tex <==
\input{header.tex}
\input{preamble/acronyms}

\graphicspath{
{images/summer_school_study/png/}
{images/summer_school_study/}
{images/summer_school_study/plots/}
{images/summer_school_study/2018/}
{images/fiber_creation/}
{images/parallel_fiber_estimation/}
{images/motor_unit_assignment/}
{images/implementation/}
{images/theory/}
{images/results/basic}
{images/results/application}
{images/results/studies}
}

\begin{document}

\newcommand{\opendihu}{OpenDiHu}
\newcommand{\Opendihu}{OpenDiHu}

\frontmatter

%\setcounter{tocdepth}{2}
\tableofcontents
%\newpage

\mainmatter

%\input{01_introduction}
%\input{02_comparative_study}

%%\chapter{Generation of Meshes for the Multiscale Models}\label{sec:generation_of_meshes_for_multiscale}
%\input{03_mesh_generation_0}
%\input{03_mesh_generation_1}
%\input{04_motor_units}
%\input{05_theory_0}
%\input{05_theory_1}
%\input{05_theory_2}
%\input{05_theory_3}

%\input{06_usage_0}
%\input{06_usage_1}

%\input{07_implementation_0}
%\input{07_implementation_1}
%\input{07_implementation_2}

%\setcounter{page}{1}
%\input{08_results_0}
%\input{08_results_1a}
\input{08_results_1b}
%\input{08_results_2a}
%\input{08_results_2b}
%\input{08_results_2c}

% consistency checks: C++ (groß), finite element method, finite elements (klein)
% fiber based electrophysiology, (dashes), multi-scale,  cross section, timestep
% diffusion -> electric conduction,  circa -> approximately, geomerty, Mu, artifical
% typos: communciation



%\chapter{Theoretic Foundations in Modeling and Solution for the Neuromuscular System}
%  - ODES: 0D Hodgkin-Huxley, Shorten
%  - PDES: general FEM, diffusion, CN
%  - multi-scale model, Godunov
%  - EMG model
%  - multi-domain in FD
%  - all mechanics
%\chapter{Extensions the Models}
% all what I have improved:
%  - Strang splitting (w/ Aaron)
%  - multidomain with FEM

%\chapter{Implementation}
%  - related works, find all other frameworks, CellML
%  - opendihu from user's perspective
%  - design choices, code etc.
%  - CellML code generator
% ----------------

% \chapter{Formulation of electrophysiology and muscle contraction}
%    - electrophysiology introduction
%    \section{State of the art}
%    - Hodgkin-Huxley, shorten, advanced models, how it gets solved
%    \section{discretization}
%    - discretization of electrophysiology, operator splitting
%    \section{Standard for formulation of models}
%    - cellml introduction
%    \section{Bidomain}
%    - EMG
%    \section{Multidomain}
%    - multidomain formulation
%    \section{Formulation of solid mechanics}
%    - basics solid mechanics framework, material modeling, 
%    
%    \section{Simulation workflow}
%    - simulation workflow of skeletal muscle
%  
% \chapter{Numerics}
%   \section{Fundamentals of the discretization}
%    \section{Finite element method}
%    - basics FEM formulation of Laplace operator and diffusion equation, boundary conditions
%    \section{Incompressible nonlinear solid mechanics}
%    - incompressibility, penalty formulation vs. mixed formulation\\
%    - governing nonlinear eq.\\
%    - jacobian
%   \section{Numerical schemes}
%    \section{time stepping schemes}
%    \section{linear system solvers}
%    \section{newton algorithm}
%  % 
% \chapter{Simulation software}
%    \section{State of the art}
%    - review on bioengineering simulation frameworks 
%    
%    \section{OpenCMISS}
%  - OpenCMISS introduction, iron zinc cmgui, unstructured\\
%  
%  - Strang splitting, solvers 1D\\
%  - improved interpolation\\
%  - parallelization, issue with 1D \\
%  - 3D parallelization strategies\\
%  - design flaws, memory\\
%    % untergliedern, z.B. schnittstellen parall etc.
%    \section{The simulation framework \emph{opendihu}}
%    - modularity of opendihu, concepts (python c++ build system)
%    \section{Overview of discretization features}
%    - feature overview, implemented equations, ansatz functions, meshes
%    \section{Input and output}
%    - file i/o parallel, i: only local data important for high parallelism, o: paraview
%    \section{In-situ visualization}
%    - in-situ
%    \section{Details on the implementation}
%    \section{Representation of structured meshes}
%    \section{Parallel data handling}
%    - data structures, petsc variables, partitioning, ghost communication
%    \section{Implementation of boundary conditions}
%    - Neumann, Dirichlet boundary conditions
%    \section{Implementation of material formulation and automatic derivation of derivatives}
%    - implementation of solid mechanics with analytic differentiation
%    
%    \section{efficient and configurable data transfer}
%    - data layout details, efficient transfer of variables between solvers
%    \section{Mapping between meshes}
%    - parallel mapping between meshes, invertability of index space represesantion
%    \section{An efficient solver to the Monodomain equation}    
%    - cellml code generator and its optimizations - openmp, simd, vc
%    \section{Details on the partitioning}
%    - fibers emg structure and partitioning
%    \section{Parallelization of the multidomain system}
%    - multidomain parallelization, reordering of matrix
%    \section{load balancing}
%    - load balancing on fiber level
% \chapter{External coupling}
%    - introduction to external coupling, precice
%    \section{coupling with FEBio}
%    \section{coupling with AceFEM}
%  

%  \chapter{An algorithm for mesh generation}
%    - introduction, need for fiber and 3d mesh
%    \section{State of the art}
%    - literature, laplace potential flow idea
%    \section{Data preprocessing}
%    - visual human dataset, methods to extract surface, approximation by spline surfaces
%    \section{Outline of the algorithm}
%    - pseudo code
%    \section{Plane mesh smoothing}
%    \section{Parallelization}
%    \section{Generation of fiber meshes}
%    - generation of muscle mesh, 3D and fibers, also in parallel
%  
% \chapter{Simulation scenarios}
%    \section{Simulation of electromyography with fiber-based formulation}
%      - scenario static-biceps-emg, composite meshes
%    \section{Simulation of electromyography with multidomain formulation}
%    \section{Muscle contraction with fiber-based formulation}
%      - fibers with contraction
%    \section{Muscle contraction with multidomain formulation}
% \chapter{Technical simulation results}
%    \section{Runtime evaluation}
%    - results and experiments, runtime, peak performance\\
%    - monodomain runtime comparison OpenCMISS opendihu
%    \section{parallel partitioning}
%    - parallel partitioning and weak scaling, opencmiss and opendihu 
%    \section{memory consumption}
%    - memory scaling OpenCMISS
% \chapter{biomechanical simulation results}
%    \section{Simulation of fatigue}
%    - monodomain, hh  shorten, fatigue effects
%    \section{Simulation of EMG}
%    - static biceps emg\\
%    - fibers with contraction\\
%    - multidomain with fat layer\\
%    - multidomain with contraction\\
%
%\part{Soft tissue robotics}
%\chapter{...}
%  - introduction, handling flexible objects, overview of different object types\\
%  - basics Lagrange formulation of cable\\
%  - cable with friction on surface\\
%  - placing cable\\
%  - peg-in-hole, with sparse grids\\
%  - simulation of 2d tissue\\
%  - gripping point estimation\\
%  
%  \cite{Maier2021}
%  
%\part{Conclusion}

% -------------- Literaturseite --------------------
\newpage

%\acsetup{pages/display=first,pages/name=true}

% Abbreviations
%\printacronyms[include-classes=abbrev,name=Abbreviations]

% Nomenclature
%\printacronyms[include-classes=nomencl,name=Nomenclature]


%\bibliography{references}{}
%\bibliographystyle{abbrv}
\printbibliography[%
  % change title
  title=Bibliography
]


% -------------- Anhang ------------
%\appendix
%\input{8_anhang.tex}

\end{document}

%\input{preambule/footer}

